A Unified and Efficient Coordinating Framework for Autonomous DBMS Tuning

Recently using machine learning (ML) based techniques to optimize modern database management systems has attracted intensive interest from both industry and academia. With an objective to tune a specific component of a DBMS (e.g., index selection, knobs tuning), the ML-based tuning agents have shown to be able to find better configurations than experienced database administrators. However, one critical yet challenging question remains unexplored -- how to make those ML-based tuning agents work collaboratively. Existing methods do not consider the dependencies among the multiple agents, and the model used by each agent only studies the effect of changing the configurations in a single component. To tune different components for DBMS, a coordinating mechanism is needed to make the multiple agents cognizant of each other. Also, we need to decide how to allocate the limited tuning budget among the agents to maximize the performance. Such a decision is difficult to make since the distribution of the reward for each agent is unknown and non-stationary. In this paper, we study the above question and present a unified coordinating framework to efficiently utilize existing ML-based agents. First, we propose a message propagation protocol that specifies the collaboration behaviors for agents and encapsulates the global tuning messages in each agent's model. Second, we combine Thompson Sampling, a well-studied reinforcement learning algorithm with a memory buffer so that our framework can allocate budget judiciously in a non-stationary environment. Our framework defines the interfaces adapted to a broad class of ML-based tuning agents, yet simple enough for integration with existing implementations and future extensions. We show that it can effectively utilize different ML-based agents and find better configurations with 1.4~14.1X speedups on the workload execution time compared with baselines.

==> revision.tex <==
\thispagestyle{empty}

\newgeometry{top=19mm, bottom=20mm, left=19mm,right=19mm}


\begin{multicols*}{2}
We thank all the reviewers for the constructive feedback.
%which can help make our paper significantly stronger.
In this cover letter, we provide our response to the major concerns of the reviewers and point to the specific sections we  revised. 
We use one extra content page  to accommodate the revisions as allowed. 
The key changes are highlighted in \textcolor{blue}{blue} for clarity in the revised paper.

%We highlight our major changes in \blue{blue} text in our rehttps://www.overleaf.com/project/63b65355cc1a053915b4bf37vision, and we provide 
\textbf{Note:} 
In this cover letter, ``RC'' refers to the required change, ``R'' refers to the reviewer, ``O'' refers to the opportunity for improvement, and ``M'' refers to the minor remark.
%As suggested, we name our framework as UniTune.

\begin{table}[H]
    \centering
    \scriptsize
    \caption{Summary of Major Modifications.}
    \vspace{-1em}
    \label{tab:modif}
    \begin{tabular}{|l|l|}
        \hline
        Modifications & Reviews \\
        \hline
        Section \ref{sec:intro}:  name the proposed framework UniTune (short for unified tune) &  R3.M2\\
        \hline
        Section \ref{sec:intro}:  update the statistics of UniTune based on revised experiments &  R3.O2, R3.O11\\
        \hline
        Section \ref{sec:opt-design}:  clarify advantages of alternating optimization over the joint &  R1.O1, R1.O6\\
        \hline
        Section \ref{sec:opt-context}: add detailed explanation for the training  of UniTune &  R1.O4\\
        \hline
         Section \ref{sec:budget-win}: explain the unit for memory buffer size &  R3.O8\\
        \hline
        Section \ref{sec:budget-win}: discuss how to decide the tuning order &  R1.O2\\
        \hline
        Section \ref{sec:exp}: use the entire workload for JOB  and add a TPC-DS workload &  R3.O5, R3.O11\\
        \hline
        Section \ref{sec:exp}: re-execute UDO using the  open-source implementation &  R4.O1\\
        \hline
         Section \ref{sec:exp-setup}: clarify the implication of  index candidate generation  &  R3.O6\\
        \hline
        Section \ref{sec:exp-setup}: explain the setting of the scale factor for reward &  R3.O4\\
        \hline
         Section \ref{sec:exp-an-time}: analyze UniTune's execution time breakdown &  R1.O4\\
        \hline
         Section \ref{sec:exp-ana-utility}: add UCB baseline &  R3.O3\\
        \hline
        Section \ref{sec:case-extend}: discuss the extension to cost-based or rule-based agents  &  R4.O2\\
        \hline
        Section \ref{exp:case-space}: add experiment varying the storage budgets &  R3.O1, R3.O2, R3.O7\\
        \hline
       
    \end{tabular}
\end{table}


\section*{Response to Meta-reviewer}

The major modifications of the manuscript are listed in Table~\ref{tab:modif}. For the required changes, we made the following modifications.

\noindent\textbf{ RC1: Re-execute UDO.} 
We re-executed UDO using the reference open-source implementation in \textcolor{blue}{Section \ref{sec:exp-end} }. 
The result and analysis show that  UDO performs worse than UniTune since its two-layer strategy causes insufficient budgets allocated on the outer agent.

\noindent\textbf{ RC2: Comparison with UCB.} 
We compared with UCB in \textcolor{blue}{Section \ref{sec:exp-ana-utility}}.
The  result and analysis show that UCB tends to explore every agent in  dissimilar contexts due to high uncertainty and it performs worse than UniTune's strategy.

\noindent\textbf{ RC3: Organization and writing requests.}
We carefully revised the manuscript and fixed the grammatical errors.

\section*{RESPONSE TO REVIEWER \#1}

\noindent\textbf{R1.O1, R1.O6:  Joint \& alternating.}
We analyzed the drawback of joint optimization in Section \ref{sec:opt-design}: \textcolor{blue}{``First, the number of evaluations needed to \ldots''} and discussed how  alternating optimization moves towards the optimum: \textcolor{blue}{``the alternating optimization essentially\ldots''} 

\noindent\textbf{R1.O2:  Dependency directions.}
We explained how UniTune explores dependency directions by different tuning orders in Section \ref{sec:budget-win}: \textcolor{blue}{``The budget allocation strategy explores different dependency directions through different tuning orders\ldots''}

\noindent\textbf{R1.O3: Query-level Tuning.} 
Our method can support query-level tuning by executing the target query when evaluating in DBMS.
Section \ref{sec:exp-case-grid} is an example of our query-level tuning result.

\noindent\textbf{R1.O4: Training of the framework.}
In Section \ref{sec:opt-context}, we  (1) clarified the training data format:  \textcolor{blue}{``the format of the training data\ldots''} and (2) emphasized that we fix the values of other agents when training:  \textcolor{blue}{``we fix the best-ever configurations\ldots''}
(3) In \textcolor{blue}{Section \ref{sec:exp-an-time}}, we analyzed UniTune's execution time breakdown.

\noindent\textbf{R1.O5: Standalone tuning.}
We clarified the definition of the standalone tuning in Section \ref{sec:exp-setup}: \textcolor{blue}{``Standalone tuning tunes a single\ldots''}


\section*{RESPONSE TO REVIEWER \#3}

\noindent\textbf{R3.O1, R3.O2, R3.O7: Storage Budget.}
 We  added an experiment varying the storage budgets for index and view in \textcolor{blue}{Section \ref{exp:case-space}}.
 The results show : \textcolor{blue}{``
For the view component, its tuning benefit saturates after being given 500MB storage budget\ldots For the index component, its tuning benefit  increases significantly from zero storage budget to 1500 MB and then the increase becomes gentle\ldots''}
As shown in the experiment, \textcolor{blue}{the tuning performance gradually increases with the given storage budget and then saturates}. 
Users should decide the storage budgets based on their affordable storage resource.



\noindent\textbf{R3.O3: Comparison with UCB.}
We compared with UCB in \textcolor{blue}{Section \ref{sec:exp-ana-utility}}.
The evaluation result and analysis show that UCB tends  to explore every agent in dissimilar contexts due to high uncertainty and performs worse than UniTune's strategy.

\noindent\textbf{R3.O4: Explanation on the scale factor for reward.}
We explained its setting in Section \ref{sec:exp}:\textcolor{blue}{``To set $rfactor$ for Algorithm \ref{alg:select}\ldots''}


\noindent\textbf{R3.O5, R3.O11: Test on Larger workloads.}
We re-executed the experiments for JOB using the 113 JOB queries and re-reported the performance in \textcolor{blue}{Figure \ref{fig:exp-end}, Figure \ref{fig:exp-ana-context}, Figure \ref{fig:exp-ana-budget1}, Figure \ref{fig:exp-case-joint}}.
We observed that the  relative tendencies are consistent with previous results of tuning JOB with 24 queries.
For TPC-H, we explained the reason for using partial queries in Section \ref{sec:exp-setup}: \textcolor{blue}{``For TPC-H, some  queries have costs orders of magnitude higher than the average value.
Including them in the workload makes the index selection problem much simpler~\cite{DBLP:journals/pvldb/KossmannHJS20} because \ldots''}
As suggested, we  added the experiment on TPC-DS with a scale factor of 50 using all the 99 queries provided in \textcolor{blue}{ Section \ref{sec:exp-end}} and UniTune still outperforms the  baselines and improves the default execution time by 2.7 hours.
Based on the revised experiments, we updated the statistics: UniTune achieves \textcolor{blue}{$1.4\times$\textasciitilde$14.1\times$} speedups on the execution time of the best configurations compared with baselines.


%\noindent Table \ref{tab:case} presents  the tuning result for a single query. 
%We added its default performance in Section \ref{sec:exp-case-grid}: \textcolor{blue}{the default performance without tuning is 581 seconds} and UniTune optimizes the performance to 27 seconds via 2.6 hours.

\noindent\textbf{R3.O6: Clarification on index candidates.}
The index candidate generation is necessary.
We  added its implication: \textcolor{blue}{``we generate index candidate set as the set of all potentially useful indexes\ldots''}
There are a total of 108 columns in JOB, 63 columns in TPC-H, and 429 columns in TPC-DS, but not all of them are indexable.

\noindent\textbf{R3.O8: Benefit of UDO on  index.}
Evaluating the benefit purely achieved by tuning index is not needed in UDO's training.
%, since UDO updates its index agent using the best performance tuned by light agents (knob, query) on the suggested index configuration.
In the revision, we presented its benefit on  index via additional evaluations.% not counting as UDO's budget in \textcolor{blue}{Figure \ref{fig:exp-end-ar}}.https://www.overleaf.com/project/63b65355cc1a053915b4bf37

\noindent\textbf{R3.O9: Units for memory buffer.}
The unit is one observation.
UniTune restricts the number of  considered  observations for the reward of selecting an agent.
We explained the unit in Section \ref{sec:budget-win}: \textcolor{blue}{``The buffer size represents the number of considered observations''}.


\noindent\textbf{R3.O10, R3.M1, R3.M2.} As suggested, we changed the figure order, corrected the name to $C^2UCB$ and named our method as UniTune.

\section*{RESPONSE TO REVIEWER \#4}

\noindent\textbf{R4.O1: Re-execute UDO.} 
We re-executed UDO using the referenced open-source implementation (including features such as reordering configurations), as declared in Section \ref{sec:exp-setup}: \textcolor{blue}{``We adopt the implementation released by the authors ~\cite{udo}\ldots''}
We updated the results in Section \ref{sec:exp-end}: \textcolor{blue}{``UDO outperforms sequential  approaches in most cases\ldots''}
However, it performs worse than UniTune since \textcolor{blue}{`` Its  two-layer schema can not flexibly invest  the tuning budget on promising agents and causes insufficient budget allocated on the outer agent (i.e., index agent)\ldots The ratio of
configurations explored by UDO on index, query, knob is fixed to
1:3:5 during tuning\ldots''}

\noindent\textbf{R4.O2: Extension to cost-based or rule-based agents.} 
As suggested, we discussed the extension to  those agents  and  added an experiment where UniTune coordinated with a rule-based agent, MysqlTuner in \textcolor{blue}{Section \ref{sec:case-extend}}.

\noindent\textbf{R4.O3: Guarantees of optimal solutions.} 
The convergence  to optimal solutions relies on the adopted tuning agents.
We discussed how UniTune moves towards the optimum in Section \ref{sec:opt-design}: \textcolor{blue}{``the alternating optimization essentially\ldots''} 

\noindent\textbf{R4.O4,R4.M1,R4.M2.}  We checked the manuscripts carefully and fixed the corresponding typos. 

\end{multicols*}


